Towards a Better Metric for Evaluating Question Generation Systems

There has always been criticism for using $n$-gram based similarity metrics, such as BLEU, NIST, etc, for evaluating the performance of NLG systems. However, these metrics continue to remain popular and are recently being used for evaluating the performance of systems which automatically generate questions from documents, knowledge graphs, images, etc. Given the rising interest in such automatic question generation (AQG) systems, it is important to objectively examine whether these metrics are suitable for this task. In particular, it is important to verify whether such metrics used for evaluating AQG systems focus on answerability of the generated question by preferring questions which contain all relevant information such as question type (Wh-types), entities, relations, etc. In this work, we show that current automatic evaluation metrics based on $n$-gram similarity do not always correlate well with human judgments about answerability of a question. To alleviate this problem and as a first step towards better evaluation metrics for AQG, we introduce a scoring function to capture answerability and show that when this scoring function is integrated with existing metrics, they correlate significantly better with human judgments. The scripts and data developed as a part of this work are made publicly available at https://github.com/PrekshaNema25/Answerability-Metric

==> backup_intro.tex <==
\section{Introduction} \label{sec:introduction}
Over the past few years, Question Answering (QA) systems have received a lot of attention leading to the development of several large scale datasets for document QA, knowledge base driven QA and Visual QA \cite{data_squad, dataset_teachingmachines,dataset_cbt,dataset_wdw,data_trivia, data_marco, dataset_newsqa, data_race}, \cite{data_kb_wikimovies, data_simpleQA} ,\cite{movieqa, VQA, data_clevr} thereby enabling the development of supervised models. However, as is always the case, data hungry neural network based solutions could benefit from even more training data, especially in specific domains which existing datasets to not cater to.  Creating newer datasets for specific domains or augmenting existing datasets with more data is a tedious, time consuming and expensive process. To alleviate this problem and create even more training data, there is growing interest in developing techniques that can automatically generate questions from a given source, say, a document \cite{learningtoask, model_where_to_focus}, knowledge graph \cite{data_kb_generation_eacl, sarath_factoid}, or image \cite{qg_vqa, qg_vae}. We refer to this task as Automatic Question Generation (AQG).

Given the practical importance of AQG and its potential to influence research in QA itself, it is quite natural to expect that there will soon be an explosive growth in the research in this area. This is already evident from the prolific work in this field in the past few months itself \cite{qg_vae,qg_vqa,qg_goaloriented,model_qg_learningtoask,model_qg_for_qa,model_joint_model_qa_qg}. We believe that before this field grows further, it is very important that the community critically examines the current evaluation metrics being used for this task. In particular, there is a need to closely examine the utility of existing $n$-gram based similarity metrics such as BLEU \cite{bleu}, METEOR \cite{meteor}, NIST \cite{nist}, \textit{etc.} which have been adapted for this task (as is typically the case for any new Natural Language Generation (NLG) task). This work is a first step in that direction where we propose that apart from \textit{$n$-gram similarity}, any metric for AQG should also take into account the \textit{answerability} of the generated questions. With the help of a few examples below, we illustrate that answerability depends on the presence of relevant information such as (Wh-types), entities, relations, \textit{etc.} and it is possible that a generated question has a high BLEU score but is still unanswerable and hence not useful.

To begin with, consider the task of answering questions from a Knowledge Graph. Let us assume that the intended (gold standard) question is ``Who was the director of Titanic ?'' and two different AQG systems generated the following questions ``S1: Who director Titanic ?'' and ``S2: Who was the  of Titanic ?''. Any $n$-gram based evaluation metric would obviously assign a much higher score to S2 (BLEU-3: $56.3$) than S1 (BLEU-3: $0$). However, as should be obvious S1 contains all the relevant information and most humans would be easily able to understand and answer this question. A good evaluation metric should capture this notion of answerability and give more importance to relevant words in the question than irrelevant words. This brings us to the question ``Which words are relevant?''

The above example might give the false impression that \textit{stop words} are not important and \textit{named entities} are very important. However, this is misleading and may not always be the case. For example, consider the case of answering questions from an image. %is there some water? vs is some water?; 
The questions ``Who is sitting \textit{in} the car ?'' and ``Who is sitting \textit{on} the car ?'' cannot be answered correctly unless the correct stop word (\textit{in, on}) is present in the question thereby indicating the importance of stop words. On the other hand, consider the task of answering questions from a passage titled ``Mahatma Gandhi''. In this case most humans will be able to answer the question ``What is the birth date of'' even though the actual named entity is missing (but the passage only talks about ``Mahatma Gandhi''). Thus, the idea of which portions of the question are important is closely tied to the source (document, knowledge graph, image) from which the question is being answered and a good AQG metric should take this into account.

To concretize the intuitions developed with the help of the above examples, we first perform human evaluations. Specifically, we take questions from existing datasets for document QA, knowledge base QA and visual QA and add systematic noise to these questions. We show these questions to humans and ask them to assign scores to these questions based on the \textit{answerability} and hence usefulness of these questions (\textit{i.e.}, whether the question contains enough information for them to be able to answer it correctly). We also compute BLEU, NIST, METEOR scores by comparing the noisy questions to the original questions and show that these metrics do not always correlate well with human judgments (in some cases the correlation is good but not in all cases). Similar studies \cite{eval_how_not_to_eval, bleu_critcs} have already shown that these metrics do not correlate well with \textit{fluency} but in this work we focus on \textit{answerability}.

Based on these human evaluations, we propose to modify existing metrics to focus on \textit{answerability} in addition to $n$-gram similarity. The idea is to make these metrics flexible so that the weight assigned to answerability and $n$-gram similarity can be adjusted depending on the task  (document QA, Knowledge-Base QA, Visual QA).%For example, if the questions are being used for pedagogical purposes then fluency may be as important as answerability. On the other hand if the questions are being used for training QA systems then fluency may not be as important.
Further, for capturing answerability itself we propose additional weights for different portions of the question such as, question type, content words, %stop words,
named entities, etc. These weights can be learned from a small amount of human evaluated data. In fact, we learn these weights using the human evaluation data mentioned above and find that these weights differ from task to task. For example, our human evaluation data suggests that while answering questions over knowledge bases humans assign more weights to named entities whereas when answering questions over images stop words are also important. We will release this data so that other researchers can build on it and perhaps propose even better evaluation metrics.

%As mentioned earlier, our work is only the first step in this direction and though it correlates better with human judgments there is clearly scope for improvement. \\

%Lastly, it is also important to check whether the performance of QA systems trained on such generated questions correlates with the goodness of these questions as measured by these metrics. Ideally, we would expect that the better the quality of the questions as indicated by these metrics, the better should be the performance of the system. On experimenting with state of the art systems for document QA, knowledge graph QA and visual QA we find that the new metric gives a better idea about whether the generated questions will be useful for training a QA system.   


==> current_aqg.tex <==

\begin{table*}
\centering
\scalebox{0.6}{%
\begin{tabular}{|p{9cm}|p{6cm}|p{6cm}|l|p{1.5cm}|}
\hline
\textbf{Sentence}                                                                                                                                                                                                                     & \textbf{Original Question}                                                                                                                       & \textbf{Generated Question}                      & \multicolumn{1}{l|}{\textbf{BLEU-4}} & \textbf{Human Rating} \\ \hline
in 1648 before the term genocide had been coined , the peace of westphalia was established to protect ethnic , national , racial and in some instances religious groups .                                       & what year was the peace of westphalia signed ?                                                & in what year was the term apartheid ? &   35.6                                 & 1            \\
\hline
in fact , in january 2005 , an international commission of inquiry on darfur , authorized by un security council resolution 1564 of 2004 , issued a report to the secretary-general stating that `` the government of the sudan has not pursued a policy of genocide . & what did un security council resolution 1564 authorize in 2004 ?                                                                                          & when was the un security council resolution issued ?     &   26.9           & 2                     \\ \hline
in the top 8 , sam woolf received the fewest votes , but he was saved from elimination by the judges .                                                                                     & which contestant was saved by the judges after getting the least votes on season 13 of american idol ? & who received the fewest votes in the top 8 ?     &   0.0          & 5                     \\
\hline
beyoncé 's husband jay z acquired the  parent company of tidal , aspiro , in the first quarter of 2015 .                                                                                 & the parent company of tidal became under the ownership of whom in 2015 ?                        & who acquired the parent company of tidal ?       &   0.0            & 5                     \\ \hline
\end{tabular}%
}
\caption{Generated questions from an exisiting AQG model \cite{learningtoask}}
\label{tab:nqg}
\end{table*}
\section{Current Question Generation Systems} \label{sec:agg}
As discussed earlier, the quality of generated questions should be quantified based on its \textit{answerability}, along with fluency and adequacy. To verify the hypothesis that the $n$-gram similarity metrics do not capture this behavior, we evaluate the quality of the questions generated by the sentence-model proposed in \cite{learningtoask}\footnote{We did not evaluate the state of the art model as the code was not available and the improvement gain is just 1 BLEU ($12.28$) point over \cite{learningtoask} . Thus the conclusions drawn will not change drastically}. The sentence-model uses encode-attend-decode paradigm to generate a question based on a given sentence. The performance of the system is evaluated using BLEU-4. We randomly sampled $200$ questions generated by this model and asked the annotators to rate the generated questions on a scale of $1-5$ based on ``How similar is the generated question to the original question in terms of answerability?''. Each generated question was rated by three annotators, and a gold-score for each question was then decided using a majority rule. Table \ref{tab:nqg} lists down some of the examples where it is very clear that BLEU-4 does not correlate with \textit{answerability}. Based on this analysis we also observed that question/answer type, content words and named entities indeed plays a crucial role in answerability, validating the intuition presented in Section \ref{sec:introduction}. Ideally we should have done the analysis with the output of current AQG systems. However, the quality is so bad that it becomes difficult to do any meaningful analysis, We observed that the average rating given to the questions is $2.3$ and $78$\% of the questions were rated $<=3$. Hence, we simulated the output of AQG systems by artificially constructing noisy questions where only one of the relevant information was dropped (\textit{i.e.}, either function words or named entities or question type and so on).



==> dataset.tex <==
\section{Datasets}
 We perform our evaluations on $3$ different QA tasks \textit{viz.} document QA (SQuAD) \cite{data_squad}, knowledge-base QA (WikiMovies) \cite{data_kb_wikimovies} and visual QA (VQA) \cite{VQA}. We now present a brief description of each of the $3$ datasets.
\subsection{SQuAD}
 Stanford Question Answering Dataset (SQuAD) \cite{data_squad} is a reading comprehension dataset consisting of questions based on passages from Wikipedia articles. The dataset consists of around 100K questions based on around 500 articles. Crowd-source workers were asked to form questions based on the passages such that the answers to the questions were part of the span from the passage. The average question length is 10 words.
\subsection{WikiMovies}
The WikiMovies \cite{data_kb_wikimovies} dataset consists of question answer pairs from the movie domain. The dataset consists of around 43K entities and around 100K question answer pairs. It consists of $9$ different relation types \textit{(director, writer, actor, release year, language, genre, tags, IMDb rating and IMDb votes)}. The questions are template-based and the average length of question is 9 words.
\subsection{VQA}
The Visual Question Answering dataset \cite{VQA} consists of open-ended questions pertaining images. The dataset contains 265,016 images with around $5.4$ questions on average per image. The questions were collected by crowd-source workers. Each question is answered by 10 annotators, thus leading to 10 ground truth answers  in natural language. The questions are divided into 21 categories, given in Table 3 of \cite{VQA}, such as ``What color'', ``What brand'', ``Is the'', \textit{etc}. The same categories are used as question types in Section 5. The average question length is 6 words. 

==> human_correlation_metrics.tex <==
\begin{table*}[!tbh]
\centering
\caption{Human-Correlation with Different Metrics for SQuAD}
\label{squad_human_co}
\begin{tabular}{|l|ll|ll|ll|ll|}
\hline
\multicolumn{1}{|c|}{\multirow{3}{*}{\textbf{Metric}}} & \multicolumn{8}{c|}{\textbf{Squad}}                                                                                                                                                 \\ \cline{2-9} 
\multicolumn{1}{|c|}{}                                 & \multicolumn{4}{c|}{\textit{Normal Metric}}                                              & \multicolumn{4}{c|}{\textit{Q-Metric}}                                                   \\ \cline{2-9} 
\multicolumn{1}{|c|}{}                                 & \textit{\textbf{Pearson}} & p-value        & \textit{\textbf{Spearman}} & p-value        & \textit{\textbf{Pearson}} & p-value        & \textit{\textbf{Spearman}} & p-value        \\ \hline
Bleu-4                                                 & 0.430                     & \textless 0.01 & 0.559                      & \textless 0.01 & 0.587                     & \textless 0.01 & 0.583                      & \textless 0.01 \\
Bleu-3                                                 & 0.403                     & \textless 0.01 & 0.581                      & \textless 0.01 & 0.572                     & \textless 0.01 & 0.606                      & \textless 0.01 \\
Bleu-2                                                 & 0.449                     & \textless 0.01 & 0.597                      & \textless 0.01 & 0.597                     & \textless 0.01 & 0.621                      & \textless 0.01 \\
Bleu-1                                                 & 0.481                     & \textless 0.01 & 0.607                      & \textless 0.01 & 0.610                     & \textless 0.01 & 0.629                      & \textless 0.01 \\
Rouge-L                                                & 0.496                     & \textless 0.01 & 0.589                      & \textless 0.01 & 0.623                     & \textless 0.01 & 0.645                      & \textless 0.01 \\
METEOR                                                & 0.572                     & \textless 0.01 & 0.578                      & \textless 0.01 & 0.634                     & \textless 0.01 & 0.609                      & \textless 0.01 \\ 
NIST                                               & 0.412                     & \textless 0.01 & 0.539                      & \textless 0.01 & 0.567                     & \textless 0.01 & 0.589                      & \textless 0.01 \\ \hline
\textbf{Human}                                                & 0.697                     & \textless 0.01 & 0.67                      & \textless 0.01 & -                     & - & -                      & - \\ \hline
\end{tabular}
\end{table*}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[!tbh]
\centering
\caption{Human-Correlation with different metrics for WikiMovies}
\label{wikimovies_hu_bleu}
\begin{tabular}{|l|llll|ll|ll|}
\hline
\multicolumn{1}{|c|}{\multirow{3}{*}{\textbf{Metric}}} & \multicolumn{8}{c|}{\textbf{WikiMovies}}                                                                                                                                                                                                                                                                                           \\ \cline{2-9} 
\multicolumn{1}{|c|}{}                                 & \multicolumn{4}{c}{\textit{Normal-Metric}}                                                                                                                          & \multicolumn{4}{c|}{\textit{Q-Metric}}                                                                                                                       \\ \cline{2-9} 
\multicolumn{1}{|c|}{}                                 & \multicolumn{1}{c}{\textit{\textbf{Pearson}}} & \multicolumn{1}{c|}{p-value}        & \multicolumn{1}{c}{\textit{\textbf{Spearman}}} & \multicolumn{1}{c|}{p-value} & \multicolumn{1}{c}{\textit{\textbf{Pearson}}} & \multicolumn{1}{c|}{p-value} & \multicolumn{1}{c}{\textit{\textbf{Spearman}}} & \multicolumn{1}{c|}{p-value} \\ \hline
Bleu-4                                                 & 0.114                                         & \multicolumn{1}{l|}{\textless 0.01} & 0.061                                           & 0.11                         & 0.744                                         & \textless 0.01               & 0.661                                          & \textless 0.01               \\
Bleu-3                                                 & 0.157                                         & \multicolumn{1}{l|}{\textless 0.01} & 0.092                                           & 0.03                         & 0.745                                         & \textless 0.01               & 0.686                                          & \textless 0.01               \\
Bleu-2                                                 & 0.187                                         & \multicolumn{1}{l|}{\textless 0.01} & 0.185                                          & \textless 0.01               & 0.745                                         & \textless 0.01               & 0.693                                          & \textless 0.01               \\
Bleu-1                                                 & 0.269                                         & \multicolumn{1}{l|}{\textless 0.01} & 0.211                                           & \textless 0.01               & 0.746                                         & \textless 0.01               & 0.694                                          & \textless 0.01               \\
Rouge-L                                                & 0.136                                         & \multicolumn{1}{l|}{\textless 0.01} & 0.053                                           & 0.23                         & 0.751                                         & \textless 0.01               & 0.682                                          & \textless 0.01               \\
METEOR                                                & 0.086                                         & \multicolumn{1}{l|}{0.29} & 0.115                                           & 0.16                         & 0.745                                         & \textless 0.01               & 0.702                                          & \textless 0.01               \\
NIST                                                & 0.222                                         & \multicolumn{1}{l|}{\textless 0.01} & 0.249                                           & \textless 0.01                        & 0.735                                         & \textless 0.01               & 0.664                                          & \textless 0.01               \\ \hline
\textbf{Human}                                                & 0.788                     & \textless 0.01 & 0.788                      & \textless 0.01 & -                     & - & -                      & - \\ \hline
\end{tabular}
\end{table*}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[!tbh]
\centering
\caption{Human-Correlation with different metrics for VQA}
\label{vqa_human_correlation}
\begin{tabular}{|l|llll|ll|ll|}
\hline
\multicolumn{1}{|c|}{\multirow{3}{*}{\textbf{Metric}}} & \multicolumn{8}{c|}{\textbf{Visual QA}}                                                                                                                                                                                                                                                                                     \\ \cline{2-9} 
\multicolumn{1}{|c|}{}                                 & \multicolumn{4}{c}{\textit{Normal-Metric}}                                                                                                                   & \multicolumn{4}{c|}{\textit{Q-Metric}}                                                                                                                       \\ \cline{2-9} 
\multicolumn{1}{|c|}{}                                 & \multicolumn{1}{c}{\textit{\textbf{Pearson}}} & \multicolumn{1}{c|}{p-value} & \multicolumn{1}{c}{\textit{\textbf{Spearman}}} & \multicolumn{1}{c|}{p-value} & \multicolumn{1}{c}{\textit{\textbf{Pearson}}} & \multicolumn{1}{c|}{p-value} & \multicolumn{1}{c}{\textit{\textbf{Spearman}}} & \multicolumn{1}{c|}{p-value} \\ \hline
Bleu-4                                                 & 0.06                                          & \multicolumn{1}{l|}{0.25}    & -0.031                                         & 0.55                         & 0.256                                         & \textless 0.01               & 0.287                                          & \textless 0.01               \\
Bleu-3                                                 & 0.016                                         & \multicolumn{1}{l|}{0.75}    & -0.013                                         & 0.79                         & 0.224                                         & \textless 0.01               & 0.258                                          & \textless 0.01               \\
Bleu-2                                                 & 0.073                                         & \multicolumn{1}{l|}{0.11}    & 0.027                                          & 0.56                         & 0.266                                         & \textless 0.01               & 0.263                                          & \textless 0.01               \\
Bleu-1                                                 & 0.121                                         & \multicolumn{1}{l|}{0.11}    & 0.063                                          & 0.18                         & 0.291                                         & \textless 0.01               & 0.296                                          & \textless 0.01               \\
Rouge-L                                                & 0.124                                         & \multicolumn{1}{l|}{0.12}    & 0.059                                          & 0.21                         & 0.341                                         & \textless 0.01               & 0.337                                          & \textless 0.01               \\ 
METEOR                                                & 0.110                                         & \multicolumn{1}{l|}{0.04}    & 0.132                                         & 0.12                         & 0.280                                         & \textless 0.01               &
0.311                                          & \textless 0.01               \\ 
NIST                                                & 0.086                                         & \multicolumn{1}{l|}{0.11}    & 0.075                                          & 0.16                         & 0.255                                         & \textless 0.01               & 
0.274                                          & \textless 0.01               \\ \hline
\textbf{Human}                                                & 0.675                     & \textless 0.01 & 0.661             & \textless 0.01 & -                     & - & -                      & - \\ \hline
\end{tabular}
\end{table*}


==> machine.tex <==
\begin{table}[!tbh]
\begin{minipage}{0.5\textwidth}
\centering
\begin{tabular}{|p{2cm}|l|l|l|}
\hline
\multicolumn{4}{|c|}{\textbf{WikiMovies Dataset}}                                                                    \\ \hline
\textbf{Perturbations} & \textbf{BLEU} & \textbf{QBLEU} & \textbf{Hit 1(\%)} \\ \hline
\textbf{Original}      & 100           &      100          & 76.5          \\ \hline
\textbf{Stop Words}            & 25.4            &    84.0            & 75.6         \\ \hline
\textbf{Relation Words}        & 29.4          &     64.3           & 54.7          \\ \hline
\textbf{Question Type}           & 74.0          &  79.3              & 73.5          \\ \hline
\textbf{NER}                   & 41.9          &     48.5           & 17.97         \\ \hline
\end{tabular}
\caption{Accuracy reported across different types of questions for WikiMovies Dataset}
\label{machine_wikimovies}
\end{minipage}
\begin{minipage}{0.5\textwidth}
\sisetup{table-format=-1.2}
\centering
\begin{tabular}{|p{2cm}|c|c|c|c|}
\hline
\multicolumn{5}{|c|}{\textbf{SQuAD Dataset}}                                                                                                                                                                                                                                   \\ \hline
\textbf{Perturbations}                & \multicolumn{1}{l|}{\textbf{BLEU}} & \multicolumn{1}{l|}{\textbf{QBLEU}} & \multicolumn{1}{l|}{\textbf{F1}} & \multicolumn{1}{l|}{\textbf{EM}} \\ \hline
\textbf{Original}                     & 100                                & 100                                    & 76.5                                 &    66.5                                                                \\ \hline
\textbf{NER}                                  & 77.0                               &  76.7                                   & 73.8                            & 54.0                                                             \\ \hline
\textbf{Question Type}                          & 80.1                               &  70.3                                   & 69.0                            & 59.7                                                       \\ \hline
\textbf{Stop Words}                           & 24.2                               & 69.59                                    & 70.4                            & 65.8                                                        \\ \hline
\textbf{Relevant Words}                      & 60.7                               &   63.4                                  & 64.1                            & 61.7                                                            \\ \hline
\end{tabular}
\caption{Accuracy reported across different types of questions for SQuAD Dataset}
\label{adv_squad}
\end{minipage}
\begin{minipage}{0.5\textwidth}
\sisetup{table-format=-1.2}
\centering
\begin{tabular}{|p{2cm}|c|c|c|}
\hline
\multicolumn{4}{|c|}{\textbf{VQA Dataset}}                                                                                                                                                                                                                             \\ \hline
\textbf{Perturbations} & \multicolumn{1}{l|}{\textbf{BLEU}} & \multicolumn{1}{l|}{\textbf{QBLEU}} &    \multicolumn{1}{l|}{\textbf{Overall(\%)}} \\ \hline
\textbf{Original}      & 100                                & 100                                     & 64.4                                 \\ \hline
\textbf{Relevant Words}           & 82.6                               &  78.8                       & 60.21 \\ \hline

\textbf{Question Type}           & 63.7                               &  66.36                                                                & 59.81 \\ \hline
\textbf{Stop Words}            & 10.8                               &  42.46                                    & 57.37                                 \\ \hline
\end{tabular}
\caption{Accuracy reported across different types of questions for VQA Dataset}
\label{machine_vqa}
\end{minipage}
\end{table}
\if 0 
\begin{subtable}{0.5\textwidth}
\centering
\sisetup{table-format=-1.2}

\end{subtable}
\end{table}
\section{Question Generation for Question Answering Systems}

As argued earlier, one important use case of automatically generating questions from text/images is to eventually use these generated questions to train a QA system. Given $k$ such questions generation systems, it is quite natural to rank them using the BLEU scores of the generated questions and assume that the accuracy will be in coorelation with the BLEU scores. We created $k$ such datasets for each kind of Question Answering task, and study the relation between the quality of the questions and performance on the QA system.

\subsection{Question Answering: Knowledge Base} For this variant of question answering we use Wikimovies dataset introduced in \cite{data_kb_wikimovies}. The dataset consists of 96K/10K/10K questions in train/dev/test split. Although the number of questions is 100K, each question is derived from one of the 13 template questions. The model stores the facts from the Knowledge Base in a key-value structured memory. It then uses this memory for reasoning to solve the Question Answering task. We used the baseline model described in the same work for our experiments. We used the code\footnote{https://github.com/facebook/MemNN/tree/master/KVmemnn} released by the authors to replicate the numbers and report them in row 1 of Table \ref{machine_wikimovies}.\\
We then created $k$ systems as described earlier, where each system corresponds to one single type of perturbation. In case of WikiMovies, we generated $4$ systems, where these corresponded to the absence of named entity,  stop words, relation-words and replacing question types respectively. Each of these was then used to train the baseline-model from scratch. We report the top-1/top-10/top-100 accuracies on the test split. Note that the questions in the test set were not perturbed.\\
The performance of the model drops drastically if named entities are removed from the question. This is because the model is unable to learn to retrieve the relevant memory cells. Removing relation words does not lead to a significant drop, as most of the times a named entity is associated with only one kind of relation to the movie. Replacing the question type doesn't have much impact on the model's performance, as for WikiMovies, the Knowledge base is simple. Most of the answers are either name of a movie or a person, thus given the relevant word and named entity in a question it is easy to infer the answer type.\\
It could be seen in Table \ref{machine_wikimovies} that for System with no stop words BLEU is not a good indication of high accuracy that the model achieves. Thus though QBLEU/BLEU indicates that the question quality is average, the model has learnt to ignore the question type information and still reach to correct answer. 
\subsection {Question Answering: Machine Comprehension}For this variant of question answering task, we use SQuAD dataset which was introduced in \cite{squad}. The dataset comprises of question/answers generated for 23215 passages which spanned across 536 Wikipedia articles. Crowdsource workers were asked to generate questions. It had 90K/10K questions in train/dev split. For the SQuAD dataset, we use the model proposed by \cite{DBLP:Bidaf}. This paper proposes a new mechanism to model interaction between query and passage. Also, a multi-level hierarchical process is proposed to represent passage at a different level of granularity. We replicated the numbers reported in the paper using the code\footnote{https://github.com/allenai/bi-att-flow} released by authors. \\
Similar to the $4$ systems generated for WikiMovies dataset, we generated $4$ variations of the dataset for this QA task also, i.e. removing stop-words, removing of named entities, removing relevant words and replacing the question words. 
For each training version, we report the F1 score, Exact Match(EM) score in Table \ref{adv_squad}. The F1 score and EM score corresponds to evaluation on validation split where the questions have not been perturbed.\\ 
We observe that dropping relevant words leads to the lowest score. This is because the sentence that contains the answer and question have high overlap, thus dropping the relevant words will make it difficult for the model to find the correct span. Dropping named entity does not have a significant effect as most of the times the passage talks refers to only a single entity (per type). \\
Here also it could be observed that BLEU score doesn't correlate well, it is lowest for model which has a high accuracy, i.e. the system that corresponds to the stop-words. Even it could be noted that for system where the question type is replaced, the BLEU score is high where as the accuracy is low. But it could be seen that QBLEU serves as a good indicator for the accuracy of the models.
%Here again, BLEU score correlates well is lowest for system which corresponds to no stop words but the same is not true of the model. QBLEU on the other hand have a fairly high score for the same, and could serve as a good indicator of accuracy.  
%QBLEU is almost correlated with the F1 score. The only exception we notice is for question type perturbations. This could be because the question/answer type is important to deciding the answer span i.e. where it should be a noun phrase, location, time etc. But while rating the questions judges weren't aware of the answers.


\subsection{Visual Question Answering}
For Visual Question Answering task we refer to Visual Question Generation dataset introduced in \cite{VQA}. The dataset consists of 248K/121K/244K questions on real images per train/dev/test split. These questions were asked across 82K/40K/81K images. Each question is answered by 10 turks, thus each question had a corresponding list of 10 ground truth answers. We used the state of the art model proposed in paper \cite{DBLP:journals/corr/Ben-younesCCT17} for the VQA dataset. This work models bilinear interaction between image and question using tensor-based Tucker decomposition. It is only focused on open-ended task, where the answers are natural language phrases.The model is trained to predict the most common answer among 10 ground truth answers.\\
We created three systems for this dataset, removing stop words, changing question type and removing relevant words. The performance for this task does not drop significantly with either of the perturbations, (reason is that the softmax is across a small set of answers and inherent bias itself is good to go (%XX cite paper).
However on removing stop words, the performance is the worst. This is due to the fact that many (get the numbers) questions belong to "Is the" "Are the" category. Removing the stop words changes the meaning of the question. In Table \ref{machin_vqa} it can be seen that the BLEU score and the overall accuracy are positively correlated. However an increase of 2 percent accuracy (from stop words to answer types) corresponds to a jump of 53.1 BLEU points. The BLEU metric though positively correlated is still unreliable. QBLEU on the other hand is both positively correlated and has comparable difference in the accuracy and the QBLEU score.

\fi 

==> new_abs.tex <==
\begin{abstract}
%A good question should contain all relevant information such as question type (Wh-types), entities, relations, \textit{etc.} 

Given the rising interest in automatically generating questions from a given source (document, knowledge graph, image, \textit{etc.}), it is important to critically examine the metrics which are currently being used for evaluating such automatic question generation systems.
Specifically, it is important to verify whether existing metrics focus on \textit{answerability} of the generated question by preferring questions which contain all relevant information such as question type (Wh-types), entities, relations, \textit{etc.}
In this work, we first perform human evaluations and show that current automatic evaluation metrics based on $n$-gram similarity do not always correlate well with human judgments about \textit{answerability} of a question. Note that, while earlier studies have shown that such metrics do not correlate well with \textit{fluency} and \textit{adequacy}, in this work we focus on \textit{answerability}.  
Finally, we propose to modify several existing metrics by adding a component to account for $answerability$ and show that with this modification all existing metrics correlate better with human judgments. 

%across three different tasks, viz., document QA, knowledge graph QA and image QA.     

%However, our experiments with QA systems involving documents, knowledge graphs and images suggests that this is not the case. 

%As is typically the case for any Natural Language Generation (NLG) task, these systems are evaluated using n-gram similarity based metrics such as BLEU, METEOR, NIST, \textit{etc}. However, these metrics do not capture the notion of \textit{answerability} of the generated question which depends on presence of  relevant information such as question type (Wh-types), entities, relations, \textit{etc.} in the generated question. In this work, we first argue the notion of answerability depends on the source from which the question is to be answered (the source could be a document, image, knowledge graph, \textit{etc.}) perform human evaluations and show that current automatic evaluation metrics (such as BLEU, METEOR, NIST, \textit{etc.}) do not correlate well with human judgments about \textit{answerability} of a generated question. Next, we experiment with state of the art QA systems and show that when such systems are trained on noisy questions, their performance is completely uncorrelated with the goodness of these questions as measured by the above metrics. Finally, we make a case for learnable  evaluation metrics which take into account the informativeness of the question and show that such a metric .

%An ideal metric for evaluating the performance of such questions generation systems should thus capture this notion of \textit{answerability} of questions. 

%However, this notion of completeness is not captured by n-gram similarity based evaluation metrics such as BLEU, METEOR, NIST, etc which are currently used for evaluating such question generation systems. 
\end{abstract}


==> sv_disagree.tex <==
\begin{table*}[!tbh]
\centering
\begin{tabular}{|p{2cm}|p{4cm}|p{4cm}|l|}
\hline
\textbf{Datasets}                    & \textbf{Original Question}                                                                                & \textbf{Modified Question}                                                                     & \textbf{\begin{tabular}[c]{@{}l@{}}User1/\\ User2 \\ Rating\end{tabular}} \\ \hline
\multirow{3}{*}{\textbf{SQuAD}}      & \begin{tabular}[c]{@{}l@{}}What language is used to\\ educate in Wales?\end{tabular}                      & \begin{tabular}[c]{@{}l@{}}What is used to educate\\ in Wales?\end{tabular}                    & 5/3                                                                       \\
                                     & \begin{tabular}[c]{@{}l@{}}When did Obama finally\\ visit Kenya?\end{tabular}                             & When did Obama Kenya?                                                                          & 1/3                                                                       \\
                                     & \begin{tabular}[c]{@{}l@{}}What language is used in \\ Chinese primary schools\\ in Malaysia\end{tabular} & \begin{tabular}[c]{@{}l@{}}What language is used in \\ Chinese primary schools in\end{tabular} & 1/3                                                                       \\ \hline
\multirow{3}{*}{\textbf{WikiMovies}} & Is that an Asian guy?                                                                                     & Is that an Asian ?                                                                             & 5/3                                                                       \\
                                     & Is it raining?                                                                                            & raining?                                                                                       & 4/1                                                                       \\
                                     & Is it daytime?                                                                                            & daytime?                                                                                       & 5/2                                                                       \\ \hline
\end{tabular}
\caption{Examples where Annotator1-Annotator2 do not agree}
\label{sv_disagree}
\end{table*}
\if 0 
\begin{figure*}[!th]
    \centering
    \includegraphics[width=0.31\textwidth]{images/hbmemnn}\hfill
    \includegraphics[width=0.31\textwidth]{images/hbsquad}\hfill
    \includegraphics[width=0.31\textwidth]{images/hbimage}
    \includegraphics[width=0.31\textwidth]{images/hqmemnn}\hfill
    \includegraphics[width=0.31\textwidth]{images/hqsquad}\hfill
    \includegraphics[width=0.31\textwidth]{images/hqimage}
    \caption{Human-Bleu\_4 Correlation across different datasets}
    \label{fig:hbbleu}
\end{figure*}
\fi


==> wikimovies_subtable.tex <==
\begin{subtable}{1\textwidth}
\centering
\begin{tabular}{|l|l|l|l|l|l|}
\hline
\multicolumn{6}{|c|}{\textbf{WikiMovies Dataset}}                                                                    \\ \hline
\textbf{Dataset Perturbations} & \textbf{BLEU} & \textbf{QBLEU} & \textbf{Hit 1} & \textbf{Hit 2} & \textbf{Hit 100} \\ \hline
\textbf{No Perturbations}      & 100           &      100          & 76.5          & 89.7          & 94.0            \\ \hline
\textbf{NER}                   & 56.6          &     55.4           & 17.97          & 29.9           & 42.7            \\ \hline
\textbf{Stop Words}            & 61.3            &    94.4            & 75.6          & 88.7          & 93.4            \\ \hline
\textbf{Relation Words}        & 81.0          &     76.5           & 54.7          & 77.7          & 86.8            \\ \hline
\textbf{Question Type}           & 71.5          &  65.4              & 73.5          & 87.1          & 92.1            \\ \hline
\end{tabular}
\caption{WikiMovies Dataset}
\label{machine_wikimovies}
\end{subtable}

%\textbf{Last word}             & 82.6                               & 65.1                                    & 78.34                                & 37.92                                 & 49.78                               & 60.21                                 \\ \hline
